Magnetic Ball Chain Robots for Cardiac Arrhythmia Treatment

This paper introduces a novel magnetic navigation system for cardiac ablation. The system is formed from two key elements: a magnetic ablation catheter consisting of a chain of spherical permanent magnets; and an actuation system comprised of two cart-mounted permanent magnets undergoing pure rotation. The catheter design enables a large magnetic content with the goal of minimizing the footprint of the actuation system for easier integration with the clinical workflow. We present a quasi-static model of the catheter, the design of the actuation units, and their control modalities. Experimental validation shows that we can use small rotating magnets (119mm diameter) to reach cardiac ablation targets while generating clinically-relevant forces. Catheter control using a joystick is compared with manual catheter control. blue While total task completion time is similar, smoother navigation is observed using the proposed robotic system. We also demonstrate that the ball chain can ablate heart tissue and generate lesions comparable to the current clinical ablation catheters.

==> sections/teleop.tex <==
% A complete control approach for the ball chain would use the model in Section \ref{sec:ball_chain} to map the desired rotation of the chain's tip onto the rotation of the external actuating magnet. Specifically, given a desired angular velocity for the tip of the chain $\pmb \omega_d$, we would find the actuation magnet's rotation ($\mb R_a$) by solving the optimization problem

% \begin{equation}
%     (\mb{p}_i^*, \mb R_i^*, \mb R_a^*), \ i \in 2, \ldots, n = \argmin_{\mb{p}_i, \mb R_i, \mb R_a} |\pmb \omega_n - \pmb \omega_d |^2 \nonumber \\
% \end{equation}

% under the constraint that the static equilibrium in (\ref{eq:statics}) is satisfied and that the balls are rigid, i.e.
% \begin{eqnarray}
%     \frac{\partial U}{\partial \mb p_i} = \frac{\partial U}{\partial \mb R_i} = 0, \forall i = 1, 2, \dots, n. \nonumber \\
%     |\mb{p}_i| > d \ \forall \ i=1,2,\dots,n.
% \end{eqnarray}
% Here $\pmb \omega_n$ is the angular velocity of the last ball of the chain expressed using the direct kinematics.

% However, from several experiments (see Section \ref{sec:experiments}), we observe that - for a significant length of the chain - its tip mostly aligns with the applied magnetic field. To show this, we report the results of the simulated model from Section \ref{sec:ball_chain} in Fig. \ref{fig:model_simulation}. We modelled a chain extending from 1 to 16 balls - same length used in the experiments in Section \ref{sec:experiments} - and applied a rotating magnetic field of intensity 5.8mT, i.e. the one computed for a magnet at the same distance of the experiments. The field direction $\hat{\mb B}$ was rotated from angle $0^\circ$, aligned with the direction of insertion of the chain, to $180^\circ$, anti-parallel to the ball chain.

% In Fig. \ref{subfig:model_error}, we report the angle between $\hat{\mb{B}}$ and $\hat{\mb m}_n$, i.e. $\angle (\hat{\mb{B}}, \hat{\mb m}_n)$ for different orientation of $\hat{\mb{B}}$ and varying the extension length of the ball chain (x axis). We see that, for a ball chain of length greater than 10 balls (represented in Fig. \ref{subfig:model_results}), the angle between its tangent ($\hat{\mb m}_n$) and the applied field is less than 1.4$^\circ$ (0.8\%). 

% In the experiments in Section \ref{sub:robotic_vs_manual}, where we show navigation inside the heart, 10 balls is the minimum chain length to reach every target. Therefore, we can confidently infer that in the operative conditions the chain tip can be assumed to align with the magnetic field \cite{Pittiglio2023b, Pittiglio2023c}.

% Using this observations, we can simplify the control architecture and assume that $\hat{\mb  m}_n = \hat{\mb B}$, i.e. the last ball's magnetic dipole aligns with the applied field $\hat{\mb B}$. As a consequence, the tangent at the tip $\hat{\mb v}$ aligns to the applied field. Therefore, a differential rotation of the applied field maps into a differential rotation of the chain's tip $\dot{\hat{\mb  v}} = \dot{\hat{\mb B}}$. 

% From the dipole model in (\ref{eq:dipole}), we can relate the rate of change of the magnetic field to the rotation of the actuating magnet's dipole as 

% \begin{equation}
%         \dot{\hat{\mb B}} = \frac{|\mb{m}_a| \mu_0}{4 \pi |\mb{r}|^3} \left(3 \hat{\mb{r}} \hat{\mb{r}}^T - I \right) \dot{\hat{\mb  m}}_a 
%      = \mb{M}(\mb r) \mb J(\pmb \phi_a) \pmb \omega_a. 
% \end{equation}
% Matrix $\mb J(\mb \phi_a)$ can be found as a series of elementary rotations of $\pmb \phi_a \in \mathbb{R}^3$ around $\mb x, \ \mb y$ and $\mb z$ (see Fig. \ref{fig:actuation_unit})

% \begin{equation}
%     \mb J(\pmb \phi_a) = \left(\begin{array}{ccc}
%         1 & 0 & -\sin(\phi_{a_1})\sin(\phi_{a_2})\\
%         0 & \cos(\phi_{a_1}) & \cos(\phi_{a_1}) \\
%         0 & -\sin(\phi_1) & -\sin(\phi_1)\cos(\phi_2)
%     \end{array} \right)
% \end{equation}
% with $\pmb \omega_a = \dot{\pmb{\phi}}_a$.

% Using the relationship between wheel and magnet rotation in (\ref{eq:wheel_magn}) and the fact that the chain's tip alings with the applied field, we can write

% \begin{equation}
% \label{eq:tip_to_wheel}
%     \dot{\hat{\mb  v}} = \eta \mb{M}(\mb r) \mb J(\pmb \phi_a) \mb{A} \pmb{\omega}_w.
% \end{equation}
% For a user command $\dot{\hat{\mb  v}}$, via a remote controller, we find the desired rotation of the omni wheels by inverting (\ref{eq:tip_to_wheel})

% \begin{equation}
%     \pmb \omega_w = \eta^{-1} \mb{A}^{-1} \mb J^{-1}(\pmb \phi_a) \mb{M}^{-1}(\mb r) \dot{\hat{\mb  v}}.
% \end{equation}

% In presence of a real-time localization modality we would impose $\mb r = \mb p_n$, i.e. measure the distance between the actuating magnet and the tip of the chain to infer the accurate orientation of the field. However, we approximate this distance as the position of the base of the chain, in lack of real-time localization. In the experiments in Section \ref{sec:experiments}, we do not notice particular limitations in using this simplifying assumption since the operator can correct this using visual clues.

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figures/model_results}
%          \caption{Shape results of the model in Section \ref{sec:ball_chain} for a chain of 10 balls while applying magnetic field of intensity 5.8mT rotating from 0$^\circ$ to 180$^\circ$, with increments of 22.5$^\circ$.}
%          \label{subfig:model_results}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figures/model_error}
%          \caption{Angle between applied field and chain tip tangent for rotation field from 0$^\circ$ to 180$^\circ$, with increments of 22.5$^\circ$ and varying chain length.}
%          \label{subfig:model_error}
%     \end{subfigure}
%     \caption{Simulation results showing the alignment of the chain's tip with the applied magnetic field.}
%     \label{fig:model_simulation}
% \end{figure}

==> sections/validation.tex <==
We performed experiments using the set up shown in Fig. \ref{fig:setup}. The robot was composed of ten N42 magnetic spheres of diameter 3.175 mm, mass 0.13 g and remanence 1.32 T. This was the smallest strong spherical permanent magnet available commercially (K\&J Magnetics, USA). Smaller and stronger custom magnets can be fabricated and used in applications which require robots with smaller diameter and higher magnetic content.

An external N52 cylindrical magnet (76.2mm diameter, 38.1mm long, 1.48 T remanence) was mounted on a 3-axis gimbal so that it could be precisely moved with respect to the ball chain robot. Magnet configurations were selected so as to produce a magnetic field in the $x-z$ plane, where gravity was aligned with the negative $z$ axis and the center line of the ball chain was directed along the positive $x$ axis. 

A webcam (C920, Logitech, US) was placed by the side of the robot and used to track its center line. The silicone sleeve was molded as combination of Ecoflex 00-30 and blue pigment (Silc Pig, Smooth-on, USA) to produce high visual contrast with the background. The robot's center line was extracted from the blue channel of the images using the \emph{active contour} and \emph{skeletonizing} operations from the Matlab Image Processing Toolbox. This data is reported as ``measured" in Fig. \ref{fig:model_validation}.

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{figures/model_validation.png}
    \caption{Experimental versus model-predicted shape of the ball chain robot \cite{Pittiglio2023d}.}
    \label{fig:model_validation}
\end{figure}

The magnet was first positioned with its magnetic dipole direction along the positive $x$ axis ($\psi = 0$), $\hat{\mb{m}}_e = e_1$ and the angle $\psi$ (see Fig. \ref{fig:setup}) increased in steps: $30^\text{o},\ 60^\text{o},\ 75^\text{o},\ 90^\text{o}$. These steps generate the four downward configurations in Fig. \ref{fig:model_validation}. This is the largest rotation we could achieve with the used gimbal. 

Next, the magnet was rotated so that its dipole direction is along the negative $x$ axis, $\hat{\mb{m}}_e = -e_1$. The angle $\psi$ was then adjusted to angles of $90^\text{o},\ 75^\text{o},\ 60^\text{o},\ 30^\text{o}$ to generate the upward motion in Fig. \ref{fig:model_validation}. An extract from the performed experiment can be found in the Supplementary Video.

The magnetic field generated by the external magnet was computed by applying the dipole model to each pose of the external magnet, as expressed in (\ref{eq:dipole}). The position of the magnet with respect to the $i$th ball magnet $\mb{p}_i$ is $\mb{r}_i = \mb{p}_e - \mb{p}_i$, with $\mb{p}_e = (v_3 - v_1 \sin(\psi)) \cdot e_1 + (v_1 \cos(\psi) - v_2) e_3$. Here, $v_1 = 15$ cm, $v_2 = 20$ cm and $v_3 = 35$ cm. 

For each configuration, the shape was computed as described in Section \ref{sec:kinematics}, and compared with the measured shape. The comparison is reported in Fig. \ref{fig:model_validation}. The mean error over all configurations and all spheres in the ball chains is $0.42\pm 0.47$mm.
